Constant-weight PIR: Single-round Keyword PIR via Constant-weight Equality Operators

Equality operators are an essential building block in tasks over secure computation such as private information retrieval. In private information retrieval (PIR), a user queries a database such that the server does not learn which element is queried. In this work, we propose \emph{equality operators for constant-weight codewords}. A constant-weight code is a collection of codewords that share the same Hamming weight. Constant-weight equality operators have a multiplicative depth that depends only on the Hamming weight of the code, not the bit-length of the elements. In our experiments, we show how these equality operators are up to 10 times faster than existing equality operators. Furthermore, we propose PIR using the constant-weight equality operator or \emph{constant-weight PIR}, which is a PIR protocol using an approach previously deemed impractical. We show that for private retrieval of large, streaming data, constant-weight PIR has a smaller communication complexity and lower runtime compared to SEALPIR and MulPIR, respectively, which are two state-of-the-art solutions for PIR. Moreover, we show how constant-weight PIR can be extended to keyword PIR. In keyword PIR, the desired element is retrieved by a unique identifier pertaining to the sought item, e.g., the name of a file. Previous solutions to keyword PIR require one or multiple rounds of communication to reduce the problem to normal PIR. We show that constant-weight PIR is the first practical single-round solution to single-server keyword PIR.

==> tables/pir-packed-parallel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[!ht]
\centering
\caption{Runtime of Constant-weight PIR executed with parallelization}
\label{tab:packed-parallel}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{\extracolsep{4pt}}cccccccccc@{}}
\toprule
&&& \multicolumn{2}{c}{Communication (KB)} & \multicolumn{4}{c}{Time (ms)} & \\ \cline{4-5}\cline{6-9}
\begin{tabular}[c]{@{}c@{}}\# DB\\Rows ($n$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}DB Size\\(MB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Encoding\\Size\end{tabular} & \begin{tabular}[c]{@{}c@{}}Query\\Comm.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Response\\Comm.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Expansion\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sel. Vec.\\Calculation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inner Product\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Server\end{tabular} & \begin{tabular}[c]{@{}c@{}}Valid\\Response\end{tabular} \\ \midrule
256 & 5.242 & 24 & 216 & 103 & 137 & 392 & 174 & 915 & \cmark \\
512 & 10.485 & 33 & 216 & 103 & 174 & 749 & 400 & 1523 & \cmark \\
1024 & 20.971 & 46 & 216 & 103 & 153 & 1545 & 770 & 2669 & \cmark \\
2048 & 41.943 & 65 & 216 & 103 & 192 & 2959 & 1688 & 5044 & \cmark \\
4096 & 83.886 & 92 & 216 & 103 & 244 & 5621 & 3083 & 9150 & \cmark \\
8192 & 167.772 & 129 & 216 & 103 & 300 & 11051 & 6483 & 18038 & \cmark \\
16384 & 335.544 & 182 & 216 & 103 & 325 & 21704 & 13094 & 35332 & \cmark \\
32768 & 671.088 & 257 & 216 & 103 & 507 & 42647 & 26456 & 69832 & \cmark \\
65536 & 1342.177 & 363 & 216 & 103 & 526 & 85765 & 50539 & 137080 & \cmark \\
131072 & 2684.354 & 513 & 216 & 103 & 948 & 172771 & 105093 & 279110 & \cmark \\
262144 & 5368.709 & 725 & 216 & 103 & 1195 & 345965 & 223047 & 570666 & \cmark \\
\bottomrule
\end{tabular}%
}
\end{table*}
